Image2Net: Datasets, Benchmark and Hybrid Framework to Convert Analog Circuit Diagrams into Netlists

Large Language Model (LLM) exhibits great potential in designing of analog integrated circuits (IC) because of its excellence in abstraction and generalization for knowledge. However, further development of LLM-based analog ICs heavily relies on textual description of analog ICs, while existing analog ICs are mostly illustrated in image-based circuit diagrams rather than text-based netlists. Converting circuit diagrams to netlists help LLMs to enrich the knowledge of analog IC. Nevertheless, previously proposed conversion frameworks face challenges in further application because of limited support of image styles and circuit elements. Up to now, it still remains a challenging task to effectively convert complex circuit diagrams into netlists. To this end, this paper constructs and opensources a new dataset with rich styles of circuit diagrams as well as balanced distribution of simple and complex analog ICs. And a hybrid framework, named Image2Net, is proposed for practical conversion from circuit diagrams to netlists. The netlist edit distance (NED) is also introduced to precisely assess the difference between the converted netlists and ground truth. Based on our benchmark, Image2Net achieves 80.77% successful rate, which is 34.62%-45.19% higher than previous works. Specifically, the proposed work shows 0.116 averaged NED, which is 62.1%-69.6% lower than state-of-the-arts. Our datasets and benchmark are available at https://github.com/LAD021/ci2n_datasets.

==> paragraphs/02_Dataset_1Definition.tex <==
We categorize 22 types of devices shown in Fig.2\ref{fig:devices_example}. Here is a description of each type: \texttt{pmos} and \texttt{nmos} represent MOS devices with no external connections to the body, while \texttt{pmos\_bulk} and \texttt{nmos\_bulk} represent MOS devices with external connections to the body. \texttt{pnp} and \texttt{npn} represent normal BJT. \texttt{pmos\_cross}, \texttt{nmos\_cross}, \texttt{pnp\_cross}, \texttt{npn\_cross} represent a device with a set of parallel Gate ports or Base ports. This type of device has two Gate/Base ports in the legend. \texttt{voltage} represents a voltage source with a circular icon, and \texttt{voltage\_lines} represents a voltage source with a striped icon. \texttt{resistor\_1} represents a resistor of the American standard, and \texttt{resistor\_2} represents a resistor of the European standard. Besides, all the other devices can be comprehended through the literal meanings of their labeled names.

\begin{figure}[ht]
  \centering
  \includegraphics[width=\linewidth]{pics/device_examples_final.png}
  \caption{\textbf{Legends for all devices}. \textbf{(a)} nmos \textbf{(b)} nmos\_cross \textbf{(c)} nmos\_bulk \textbf{(d)} pmos \textbf{(e)} pmos\_cross \textbf{(f)} pmos\_bulk \textbf{(g)} npn \textbf{(h)} npn\_cross \textbf{(i)} pnp \textbf{(j)} pnp\_cross \textbf{(k)} siso\_amp \textbf{(l)} diso\_amp \textbf{(m)} dido\_amp \textbf{(n)} diode \textbf{(o)} current \textbf{(p)} voltage \textbf{(q)} voltage\_lines \textbf{(r)} resistor\_1 \textbf{(s)} resistor\_2  \textbf{(t)} capacitor \textbf{(u)} inductor \textbf{(v)} gnd
}

\label{fig:devices_example}
\end{figure}

For crossings, as is shown in Fig.\ref{fig:crossings_example}, in general, there are 3 basic styles of symbols for annotating crossings: \texttt{Bridge}, \texttt{Flat}, \texttt{Dot}. Of which types of work as jumpers in a specified diagram, there are several legitimate styles which we have classified:

\begin{itemize}
\item{If any \texttt{Bridge} is found, the \texttt{Bridge} should act as a jumper, and the other symbols of the crossing are to indicate the connection of related wires.}
\item{If there are no \texttt{Bridge} and both \texttt{Dot} and \texttt{Flat} are found, the \texttt{Flat} represents jumper.}
\item{Otherwise, no jumper is found}.
\end{itemize}

\begin{figure}[!t]
\centering
%\includegraphics[width=3in]{fig5}
\subfloat[Bridge]{
		\includegraphics[width=0.1\textwidth]{pics/cross/cross1.png}}
\subfloat[Dot]{
		\includegraphics[width=0.1\textwidth]{pics/cross/cross2.png}}
\subfloat[Flat]{
		\includegraphics[width=0.1\textwidth]{pics/cross/cross3.png}}
\caption{Three types of crossings.}
\label{fig:crossings_example}
\end{figure}



==> paragraphs/03_Method_1Device.tex <==



==> paragraphs/05_Discussion.tex <==
At present, our algorithm does not take the names of devices and ports into account, nor does it handle the connections represented by the same name network. Our datasets, benchmark, and framework are all for graphically adjacent connections. To complete this step, it is necessary to consider the text information in the images and their relationship with each device and port through optical character recognition (OCR). We only processe the ground device and connecte all the networks related to it. 
Our algorithm considers the diverse styles of devices, cross-line styles, and image background styles as much as possible, but requires the image style to be standard. Some cross-line styles of images are ambiguous themselves and it is necessary to determine whether they are cross-lines through expert knowledge. Such problems may be solved by accumulating sufficient images and netlists through our method and training a multimodal large model and relying on its comprehension ability.

